Using Gamma-Ray Imaging to Measure Nuclear Lifetimes in the GRETINA Detector

GRETA, the Gamma-Ray Energy Tracking Array, is an array of highly-segmented HPGe detectors designed to track gamma-rays emitted in beam-physics experiments. Its high detection efficiency and state-of-the-art position resolution make it well-suited for imaging applications. In this paper, we use simulated imaging data to illustrate how imaging can be applied to nuclear lifetime measurments. This approach can offer multiple benefits over traditional lifetime techniques such as RDM.

==> figures/data_tables.tex <==
\begin{table}[p]
\centering 
\begin{tabular}{c c c c}
\textbf{\# of Samples} & \textbf{$ \sigma_{img} $ = 1.0 mm} & \textbf{$ \sigma_{img} $ = 2.5 mm} & \textbf{$ \sigma_{img} $ = 5.0 mm} \\ [0.5ex]
\hline
100 & 0.6307 \textpm{} 0.1592 & 0.6317 \textpm{} 0.1669 & 0.6391 \textpm{} 0.1952 \\
250 & 0.8034 \textpm{} 0.0975 & 0.8012 \textpm{} 0.0960 & 0.7985 \textpm{} 0.1009 \\
500 & 0.9788 \textpm{} 0.1053 & 0.9733 \textpm{} 0.1026 & 0.9647 \textpm{} 0.0976 \\
750 & \textbf{0.9637 \textpm{} 0.0644} & \textbf{0.9596 \textpm{} 0.0650} & \textbf{0.9549 \textpm{} 0.0667} \\
1000 & 0.9352 \textpm{} 0.0535 & 0.9332 \textpm{} 0.0542 & 0.9312 \textpm{} 0.0551 \\
1250 & 0.9225 \textpm{} 0.0468 & 0.9204 \textpm{} 0.0463 & 0.9178 \textpm{} 0.0471 \\
1500 & 0.9112 \textpm{} 0.0432 & 0.9099 \textpm{} 0.0435 & 0.9081 \textpm{} 0.0437 \\
2000 & 0.8992 \textpm{} 0.0373 & 0.8982 \textpm{} 0.0377 & 0.8959 \textpm{} 0.0377 \\
2500 & 0.8887 \textpm{} 0.0319 & 0.8873 \textpm{} 0.0318 & 0.8859 \textpm{} 0.0320 \\
3000 & 0.8849 \textpm{} 0.0290 & 0.8837 \textpm{} 0.0289 & 0.8824 \textpm{} 0.0290 \\
4000 & 0.8777 \textpm{} 0.0242 & 0.8766 \textpm{} 0.0242 & 0.8753 \textpm{} 0.0242 \\
5000 & 0.8741 \textpm{} 0.0229 & 0.8730 \textpm{} 0.0230 & 0.8723 \textpm{} 0.0232 \\
7500 & 0.8674 \textpm{} 0.0181 & 0.8662 \textpm{} 0.0182 & 0.8655 \textpm{} 0.0184 \\
10000 & 0.8651 \textpm{} 0.0157 & 0.8643 \textpm{} 0.0158 & 0.8637 \textpm{} 0.0161 \\
12500 & 0.8637 \textpm{} 0.0135 & 0.8628 \textpm{} 0.0136 & 0.8623 \textpm{} 0.0135 \\
15000 & 0.8617 \textpm{} 0.0128 & 0.8611 \textpm{} 0.0128 & 0.8606 \textpm{} 0.0130 \\
20000 & 0.8606 \textpm{} 0.0106 & 0.8599 \textpm{} 0.0105 & 0.8596 \textpm{} 0.0106 \\
25000 & 0.8593 \textpm{} 0.0098 & 0.8587 \textpm{} 0.0099 & 0.8583 \textpm{} 0.0099 \\
30000 & 0.8593 \textpm{} 0.0088 & 0.8587 \textpm{} 0.0088 & 0.8583 \textpm{} 0.0089 \\
40000 & 0.8587 \textpm{} 0.0077 & 0.8582 \textpm{} 0.0077 & 0.8578 \textpm{} 0.0078 \\
50000 & 0.8584 \textpm{} 0.0070 & 0.8578 \textpm{} 0.0070 & 0.8575 \textpm{} 0.0070 \\
\hline
\end{tabular}
\captionof{figure}{Simulated Lifetime Measurement Results, $ \sigma_{img} $ = 1.0 mm to 5.0 mm}
$ \tau_0 $ = 0.859 ns, $ \beta $ = 0.3c, $ N_{trials} $ = 1000, $ N_{samples} $ = 100 to 50K \\
Values are given in ns
\label{table:sim_lifetimes_1.0mm_to_5.0mm__100_to_50Ksamples}
\end{table}
 
\begin{table}[ht]
\centering 
\begin{tabular}{c c c c}
\textbf{\# of Samples} & \textbf{$ \sigma_{img} $ = 7.5 mm} & \textbf{$ \sigma_{img} $ = 10.0 mm} & \textbf{$ \sigma_{img} $ = 12.5 mm} \\ [0.5ex]
\hline
100 & 0.6577 \textpm{} 0.2344 & 0.6902 \textpm{} 0.2711 & 0.7232 \textpm{} 0.2942 \\
250 & 0.7937 \textpm{} 0.1014 & 0.7889 \textpm{} 0.1034 & 0.7842 \textpm{} 0.1053 \\
500 & 0.9604 \textpm{} 0.0984 & 0.9522 \textpm{} 0.0959 & 0.9471 \textpm{} 0.0960 \\
750 & \textbf{0.9503 \textpm{} 0.0677} & \textbf{0.9486 \textpm{} 0.0696} & \textbf{0.9438 \textpm{} 0.0708} \\
1000 & 0.9291 \textpm{} 0.0556 & 0.9262 \textpm{} 0.0563 & 0.9254 \textpm{} 0.0570 \\
1250 & 0.9163 \textpm{} 0.0478 & 0.9150 \textpm{} 0.0489 & 0.9128 \textpm{} 0.0493 \\
1500 & 0.9064 \textpm{} 0.0436 & 0.9046 \textpm{} 0.0441 & 0.9032 \textpm{} 0.0453 \\
2000 & 0.8956 \textpm{} 0.0381 & 0.8932 \textpm{} 0.0383 & 0.8929 \textpm{} 0.0386 \\
2500 & 0.8848 \textpm{} 0.0320 & 0.8833 \textpm{} 0.0324 & 0.8826 \textpm{} 0.0329 \\
3000 & 0.8806 \textpm{} 0.0293 & 0.8800 \textpm{} 0.0302 & 0.8796 \textpm{} 0.0304 \\
4000 & 0.8746 \textpm{} 0.0247 & 0.8738 \textpm{} 0.0254 & 0.8729 \textpm{} 0.0255 \\
5000 & 0.8717 \textpm{} 0.0236 & 0.8707 \textpm{} 0.0237 & 0.8704 \textpm{} 0.0243 \\
7500 & 0.8650 \textpm{} 0.0186 & 0.8645 \textpm{} 0.0188 & 0.8638 \textpm{} 0.0190 \\
10000 & 0.8632 \textpm{} 0.0164 & 0.8628 \textpm{} 0.0165 & 0.8625 \textpm{} 0.0171 \\
12500 & 0.8619 \textpm{} 0.0137 & 0.8616 \textpm{} 0.0138 & 0.8612 \textpm{} 0.0138 \\
15000 & 0.8602 \textpm{} 0.0132 & 0.8599 \textpm{} 0.0135 & 0.8596 \textpm{} 0.0137 \\
20000 & 0.8592 \textpm{} 0.0108 & 0.8590 \textpm{} 0.0109 & 0.8588 \textpm{} 0.0111 \\
25000 & 0.8581 \textpm{} 0.0100 & 0.8578 \textpm{} 0.0102 & 0.8577 \textpm{} 0.0104 \\
30000 & 0.8581 \textpm{} 0.0090 & 0.8579 \textpm{} 0.0092 & 0.8578 \textpm{} 0.0093 \\
40000 & 0.8576 \textpm{} 0.0079 & 0.8574 \textpm{} 0.0080 & 0.8573 \textpm{} 0.0081 \\
50000 & 0.8573 \textpm{} 0.0071 & 0.8571 \textpm{} 0.0072 & 0.8569 \textpm{} 0.0073 \\
\hline
\end{tabular}
\captionof{figure}{Simulated Lifetime Measurement Results, $ \sigma_{img} $ = 7.5 mm to 12.5 mm}
$ \tau_0 $ = 0.859 ns, $ \beta $ = 0.3c, $ N_{trials} $ = 1000, $ N_{samples} $ = 100 to 50K
\label{table:sim_lifetimes_7.5mm_to_12.5mm__100_to_50Ksamples}
\end{table}

\begin{table}[ht]
\centering 
\begin{tabular}{c c c c}
\textbf{\# of Samples} & \textbf{$ \sigma_{img} $ = 15.0 mm} & \textbf{$ \sigma_{img} $ = 20.0 mm} & \textbf{$ \sigma_{img} $ = 25.0 mm} \\ [0.5ex]
\hline
100 & 0.7789 \textpm{} 0.3088 & 0.8762 \textpm{} 0.2816 & 0.9166 \textpm{} 0.2600 \\
250 & 0.7789 \textpm{} 0.1056 & 0.7703 \textpm{} 0.1144 & 0.7648 \textpm{} 0.1262 \\
500 & 0.9405 \textpm{} 0.0972 & 0.9326 \textpm{} 0.1027 & 0.9243 \textpm{} 0.1043 \\
750 & \textbf{0.9447 \textpm{} 0.0756} & \textbf{0.9387 \textpm{} 0.0771} & \textbf{0.9370 \textpm{} 0.0833} \\
1000 & 0.9237 \textpm{} 0.0586 & 0.9222 \textpm{} 0.0616 & 0.9196 \textpm{} 0.0636 \\
1250 & 0.9120 \textpm{} 0.0508 & 0.9096 \textpm{} 0.0532 & 0.9065 \textpm{} 0.0564 \\
1500 & 0.9017 \textpm{} 0.0453 & 0.8996 \textpm{} 0.0480 & 0.8962 \textpm{} 0.0491 \\
2000 & 0.8912 \textpm{} 0.0395 & 0.8885 \textpm{} 0.0403 & 0.8868 \textpm{} 0.0427 \\
2500 & 0.8819 \textpm{} 0.0336 & 0.8803 \textpm{} 0.0351 & 0.8776 \textpm{} 0.0360 \\
3000 & 0.8781 \textpm{} 0.0311 & 0.8761 \textpm{} 0.0327 & 0.8744 \textpm{} 0.0343 \\
4000 & 0.8721 \textpm{} 0.0258 & 0.8708 \textpm{} 0.0271 & 0.8689 \textpm{} 0.0283 \\
5000 & 0.8697 \textpm{} 0.0250 & 0.8679 \textpm{} 0.0259 & 0.8666 \textpm{} 0.0274 \\
7500 & 0.8632 \textpm{} 0.0192 & 0.8620 \textpm{} 0.0203 & 0.8608 \textpm{} 0.0214 \\
10000 & 0.8619 \textpm{} 0.0173 & 0.8611 \textpm{} 0.0178 & 0.8599 \textpm{} 0.0189 \\
12500 & 0.8607 \textpm{} 0.0142 & 0.8600 \textpm{} 0.0146 & 0.8592 \textpm{} 0.0154 \\
15000 & 0.8592 \textpm{} 0.0138 & 0.8588 \textpm{} 0.0143 & 0.8578 \textpm{} 0.0152 \\
20000 & 0.8585 \textpm{} 0.0113 & 0.8580 \textpm{} 0.0118 & 0.8574 \textpm{} 0.0124 \\
25000 & 0.8575 \textpm{} 0.0105 & 0.8570 \textpm{} 0.0108 & 0.8566 \textpm{} 0.0115 \\
30000 & 0.8576 \textpm{} 0.0095 & 0.8571 \textpm{} 0.0100 & 0.8567 \textpm{} 0.0106 \\
40000 & 0.8571 \textpm{} 0.0082 & 0.8567 \textpm{} 0.0085 & 0.8564 \textpm{} 0.0089 \\
50000 & 0.8568 \textpm{} 0.0074 & 0.8565 \textpm{} 0.0077 & 0.8562 \textpm{} 0.0081 \\
\hline
\end{tabular}
\captionof{figure}{Simulated Lifetime Measurement Results, $ \sigma_{img} $ = 15.0 mm to 25.0 mm}
$ \tau_0 $ = 0.859 ns, $ \beta $ = 0.3c, $ N_{trials} $ = 1000, $ N_{samples} $ = 100 to 50K
\label{table:sim_lifetimes_15.0mm_to_25.0mm__100_to_50Ksamples}
\end{table}

\begin{table}[ht]
\centering 
\begin{tabular}{c c c c}
\textbf{\# of Samples} & \textbf{$ \sigma_{img} $ = 30.0 mm} & \textbf{$ \sigma_{img} $ = 35.0 mm} & \textbf{$ \sigma_{img} $ = 40.0 mm} \\ [0.5ex]
\hline 
100 & 0.9292 \textpm{} 0.2802 & 0.9403 \textpm{} 0.3105 & 0.9518 \textpm{} 0.3406 \\
250 & 0.7596 \textpm{} 0.1359 & 0.7543 \textpm{} 0.1462 & 0.7508 \textpm{} 0.1600 \\
500 & 0.9201 \textpm{} 0.1121 & 0.9192 \textpm{} 0.1203 & 0.9173 \textpm{} 0.1336 \\
750 & 0.9367 \textpm{} 0.0886 & 0.9361 \textpm{} 0.0939 & 0.9373 \textpm{} 0.0994 \\
1000 & \textbf{0.9171 \textpm{} 0.0677} & \textbf{0.9138 \textpm{} 0.0714} & \textbf{0.9094 \textpm{} 0.0765} \\
1250 & 0.9031 \textpm{} 0.0591 & 0.9012 \textpm{} 0.0631 & 0.8965 \textpm{} 0.0679 \\
1500 & 0.8937 \textpm{} 0.0527 & 0.8900 \textpm{} 0.0558 & 0.8860 \textpm{} 0.0601 \\
2000 & 0.8840 \textpm{} 0.0451 & 0.8815 \textpm{} 0.0474 & 0.8778 \textpm{} 0.0508 \\
2500 & 0.8757 \textpm{} 0.0388 & 0.8734 \textpm{} 0.0411 & 0.8695 \textpm{} 0.0451 \\
3000 & 0.8715 \textpm{} 0.0363 & 0.8684 \textpm{} 0.0384 & 0.8649 \textpm{} 0.0417 \\
4000 & 0.8666 \textpm{} 0.0304 & 0.8640 \textpm{} 0.0325 & 0.8608 \textpm{} 0.0345 \\
5000 & 0.8644 \textpm{} 0.0291 & 0.8621 \textpm{} 0.0309 & 0.8598 \textpm{} 0.0326 \\
7500 & 0.8593 \textpm{} 0.0225 & 0.8575 \textpm{} 0.0238 & 0.8552 \textpm{} 0.0253 \\
10000 & 0.8589 \textpm{} 0.0202 & 0.8576 \textpm{} 0.0216 & 0.8557 \textpm{} 0.0228 \\
12500 & 0.8582 \textpm{} 0.0163 & 0.8570 \textpm{} 0.0175 & 0.8558 \textpm{} 0.0188 \\
15000 & 0.8568 \textpm{} 0.0160 & 0.8559 \textpm{} 0.0172 & 0.8548 \textpm{} 0.0186 \\
20000 & 0.8568 \textpm{} 0.0131 & 0.8561 \textpm{} 0.0140 & 0.8551 \textpm{} 0.0152 \\
25000 & 0.8560 \textpm{} 0.0123 & 0.8553 \textpm{} 0.0132 & 0.8547 \textpm{} 0.0143 \\
30000 & 0.8561 \textpm{} 0.0113 & 0.8554 \textpm{} 0.0121 & 0.8545 \textpm{} 0.0129 \\
40000 & 0.8560 \textpm{} 0.0095 & 0.8556 \textpm{} 0.0100 & 0.8550 \textpm{} 0.0107 \\
50000 & 0.8558 \textpm{} 0.0085 & 0.8554 \textpm{} 0.0090 & 0.8549 \textpm{} 0.0096 \\
\hline
\end{tabular}
\captionof{figure}{Simulated Lifetime Measurement Results, $ \sigma_{img} $ = 30.0 mm to 40.0 mm}
$ \tau_0 $ = 0.859 ns, $ \beta $ = 0.3c, $ N_{trials} $ = 1000, $ N_{samples} $ = 100 to 50K
\label{table:sim_lifetimes_30.0mm_to_40.0mm__100_to_50Ksamples}
\end{table}
 
\begin{table}[ht]
\centering 
\begin{tabular}{c c c c}
\textbf{\# of Samples} & \textbf{$ \sigma_{img} $ = 45.0 mm} & \textbf{$ \sigma_{img} $ = 50.0 mm} & \textbf{$ \sigma_{img} $ = 55.0 mm} \\ [0.5ex]
\hline
100 & 0.9661 \textpm{} 0.3797 & 0.9812 \textpm{} 0.4264 & 0.9973 \textpm{} 0.4812 \\
250 & 0.7578 \textpm{} 0.1861 & 0.7674 \textpm{} 0.2250 & 0.7853 \textpm{} 0.2658 \\
500 & 0.9235 \textpm{} 0.1526 & 0.9364 \textpm{} 0.1752 & 0.9505 \textpm{} 0.2019 \\
750 & 0.9354 \textpm{} 0.1030 & 0.9352 \textpm{} 0.1109 & 0.9303 \textpm{} 0.1224 \\
1000 & \textbf{0.9076 \textpm{} 0.0820} & 0.9005 \textpm{} 0.0884 & 0.8942 \textpm{} 0.0970 \\
1250 & 0.8926 \textpm{} 0.0743 & \textbf{0.8862 \textpm{} 0.0786} & \textbf{0.8794 \textpm{} 0.0843} \\
1500 & 0.8802 \textpm{} 0.0637 & 0.8744 \textpm{} 0.0683 & 0.8667 \textpm{} 0.0726 \\
2000 & 0.8729 \textpm{} 0.0538 & 0.8672 \textpm{} 0.0586 & 0.8596 \textpm{} 0.0618 \\
2500 & 0.8653 \textpm{} 0.0476 & 0.8601 \textpm{} 0.0514 & 0.8548 \textpm{} 0.0559 \\
3000 & 0.8613 \textpm{} 0.0443 & 0.8561 \textpm{} 0.0486 & 0.8510 \textpm{} 0.0525 \\
4000 & 0.8572 \textpm{} 0.0372 & 0.8535 \textpm{} 0.0400 & 0.8483 \textpm{} 0.0422 \\
5000 & 0.8568 \textpm{} 0.0348 & 0.8530 \textpm{} 0.0379 & 0.8482 \textpm{} 0.0406 \\
7500 & 0.8525 \textpm{} 0.0271 & 0.8497 \textpm{} 0.0290 & 0.8462 \textpm{} 0.0313 \\
10000 & 0.8539 \textpm{} 0.0245 & 0.8512 \textpm{} 0.0268 & 0.8483 \textpm{} 0.0292 \\
12500 & 0.8542 \textpm{} 0.0201 & 0.8522 \textpm{} 0.0217 & 0.8496 \textpm{} 0.0235 \\
15000 & 0.8535 \textpm{} 0.0201 & 0.8513 \textpm{} 0.0211 & 0.8494 \textpm{} 0.0225 \\
20000 & 0.8543 \textpm{} 0.0164 & 0.8527 \textpm{} 0.0175 & 0.8509 \textpm{} 0.0190 \\
25000 & 0.8536 \textpm{} 0.0154 & 0.8526 \textpm{} 0.0167 & 0.8510 \textpm{} 0.0181 \\
30000 & 0.8537 \textpm{} 0.0139 & 0.8528 \textpm{} 0.0150 & 0.8516 \textpm{} 0.0163 \\
40000 & 0.8545 \textpm{} 0.0116 & 0.8537 \textpm{} 0.0126 & 0.8530 \textpm{} 0.0137 \\
50000 & 0.8544 \textpm{} 0.0104 & 0.8537 \textpm{} 0.0112 & 0.8528 \textpm{} 0.0121 \\
\hline
\end{tabular}
\captionof{figure}{Simulated Lifetime Measurement Results, $ \sigma_{img} $ = 45.0 mm to 55.0 mm}
$ \tau_0 $ = 0.859 ns, $ \beta $ = 0.3c, $ N_{trials} $ = 1000, $ N_{samples} $ = 100 to 50K
\label{table:sim_lifetimes_45.0mm_to_55.0mm__100_to_50Ksamples}
\end{table}

\begin{table}[ht]
\centering 
\begin{tabular}{c c c}
\textbf{\# of Samples} & \textbf{$ \sigma_{img} $ = 60.0 mm} & \textbf{$ \sigma_{img} $ = 65.0 mm} \\ [0.5ex]
\hline
100 & 1.0140 \textpm{} 0.5334 & 1.0317 \textpm{} 0.5894 \\
250 & 0.8275 \textpm{} 0.3685 & 0.8726 \textpm{} 0.4793 \\
500 & 0.9635 \textpm{} 0.2193 & 0.9884 \textpm{} 0.2453 \\
750 & 0.9266 \textpm{} 0.1324 & 0.9209 \textpm{} 0.1427 \\
1000 & 0.8869 \textpm{} 0.1014 & 0.8762 \textpm{} 0.1071 \\
1250 & 0.8706 \textpm{} 0.0903 & 0.8648 \textpm{} 0.0980 \\
1500 & \textbf{0.8597 \textpm{} 0.0770} & \textbf{0.8491 \textpm{} 0.0818} \\
2000 & 0.8513 \textpm{} 0.0658 & 0.8429 \textpm{} 0.0705 \\
2500 & 0.8475 \textpm{} 0.0602 & 0.8409 \textpm{} 0.0654 \\
3000 & 0.8444 \textpm{} 0.0554 & 0.8371 \textpm{} 0.0595 \\
4000 & 0.8428 \textpm{} 0.0454 & 0.8365 \textpm{} 0.0493 \\
5000 & 0.8432 \textpm{} 0.0440 & 0.8372 \textpm{} 0.0468 \\
7500 & 0.8420 \textpm{} 0.0337 & 0.8380 \textpm{} 0.0364 \\
10000 & 0.8449 \textpm{} 0.0309 & 0.8414 \textpm{} 0.0326 \\
12500 & 0.8473 \textpm{} 0.0256 & 0.8442 \textpm{} 0.0278 \\
15000 & 0.8469 \textpm{} 0.0245 & 0.8443 \textpm{} 0.0262 \\
20000 & 0.8487 \textpm{} 0.0206 & 0.8465 \textpm{} 0.0223 \\
25000 & 0.8494 \textpm{} 0.0196 & 0.8479 \textpm{} 0.0210 \\
30000 & 0.8501 \textpm{} 0.0177 & 0.8486 \textpm{} 0.0192 \\
40000 & 0.8521 \textpm{} 0.0149 & 0.8514 \textpm{} 0.0160 \\
50000 & 0.8520 \textpm{} 0.0133 & 0.8518 \textpm{} 0.0144 \\
\hline
\end{tabular}
\captionof{figure}{Simulated Lifetime Measurement Results, $ \sigma_{img} $ = 60.0 mm to 65.0 mm}
$ \tau_0 $ = 0.859 ns, $ \beta $ = 0.3c, $ N_{trials} $ = 1000, $ N_{samples} $ = 100 to 50K
\label{table:sim_lifetimes_60.0mm_to_65.0mm__100_to_50Ksamples}
\end{table}

\begin{table}[ht]
\centering 
\begin{tabular}{c c c}
\textbf{\# of Samples} & \textbf{$ \sigma_{img} $ = 70.0 mm} & \textbf{$ \sigma_{img} $ = 75.0 mm} \\ [0.5ex]
\hline
100 & 1.0468 \textpm{} 0.6484 & 1.0468 \textpm{} 0.6785 \\
250 & 0.9376 \textpm{} 0.6018 & 1.0284 \textpm{} 0.7160 \\
500 & 1.0060 \textpm{} 0.2580 & 1.0345 \textpm{} 0.2980 \\
750 & 0.9183 \textpm{} 0.1556 & 0.9181 \textpm{} 0.1727 \\
1000 & 0.8691 \textpm{} 0.1210 & 0.8605 \textpm{} 0.1245 \\
1250 & 0.8560 \textpm{} 0.1045 & 0.8493 \textpm{} 0.1129 \\
1500 & 0.8377 \textpm{} 0.0891 & 0.8258 \textpm{} 0.0960 \\
2000 & \textbf{0.8354 \textpm{} 0.0763} & \textbf{0.8268 \textpm{} 0.0801} \\
2500 & 0.8313 \textpm{} 0.0700 & 0.8239 \textpm{} 0.0729 \\
3000 & 0.8301 \textpm{} 0.0634 & 0.8221 \textpm{} 0.0674 \\
4000 & 0.8296 \textpm{} 0.0523 & 0.8214 \textpm{} 0.0565 \\
5000 & 0.8311 \textpm{} 0.0500 & 0.8237 \textpm{} 0.0537 \\
7500 & 0.8323 \textpm{} 0.0389 & 0.8263 \textpm{} 0.0415 \\
10000 & 0.8373 \textpm{} 0.0356 & 0.8331 \textpm{} 0.0386 \\
12500 & 0.8410 \textpm{} 0.0300 & 0.8380 \textpm{} 0.0321 \\
15000 & 0.8415 \textpm{} 0.0284 & 0.8397 \textpm{} 0.0304 \\
20000 & 0.8447 \textpm{} 0.0241 & 0.8444 \textpm{} 0.0260 \\
25000 & 0.8471 \textpm{} 0.0223 & 0.8464 \textpm{} 0.0242 \\
30000 & 0.8484 \textpm{} 0.0209 & 0.8482 \textpm{} 0.0225 \\
40000 & 0.8514 \textpm{} 0.0176 & 0.8512 \textpm{} 0.0191 \\
50000 & 0.8518 \textpm{} 0.0157 & 0.8519 \textpm{} 0.0171 \\
\hline
\end{tabular}
\captionof{figure}{Simulated Lifetime Measurement Results, $ \sigma_{img} $ = 70.0 mm to 75.0 mm}
$ \tau_0 $ = 0.859 ns, $ \beta $ = 0.3c, $ N_{trials} $ = 1000, $ N_{samples} $ = 100 to 50K
\label{table:sim_lifetimes_70.0mm_to_75.0mm__100_to_50Ksamples}
\end{table}

\begin{table}[ht]
\centering 
\begin{tabular}{c c c c}
\textbf{$ \tau_{0,known} $ (ns)} & \textbf{$ \sigma_{img} $ = 5.0 mm} & \textbf{$ \sigma_{img} $ = 10.0 mm} & \textbf{$ \sigma_{img} $ = 25.0 mm} \\ [0.5ex]
\hline
0.029 & \textbf{0.0291 \textpm{} 0.0008} & \textbf{0.0292 \textpm{} 0.0016} & 0.0295 \textpm{} 0.0041 \\
0.072 & 0.0728 \textpm{} 0.0013 & 0.0730 \textpm{} 0.0018 & \textbf{0.0738 \textpm{} 0.0039} \\
0.143 & 0.1452 \textpm{} 0.0023 & 0.1454 \textpm{} 0.0026 & 0.1463 \textpm{} 0.0041 \\
0.215 & 0.2191 \textpm{} 0.0035 & 0.2193 \textpm{} 0.0038 & 0.2201 \textpm{} 0.0049 \\
0.286 & 0.2926 \textpm{} 0.0048 & 0.2927 \textpm{} 0.0050 & 0.2935 \textpm{} 0.0061 \\
0.358 & 0.3675 \textpm{} 0.0061 & 0.3673 \textpm{} 0.0063 & 0.3677 \textpm{} 0.0073 \\
0.430 & 0.4408 \textpm{} 0.0073 & 0.4408 \textpm{} 0.0076 & 0.4399 \textpm{} 0.0086 \\
0.687 & 0.6996 \textpm{} 0.0144 & 0.6985 \textpm{} 0.0145 & 0.6960 \textpm{} 0.0167 \\
0.859 & 0.8723 \textpm{} 0.0232 & 0.8707 \textpm{} 0.0237 & 0.8666 \textpm{} 0.0274 \\
1.074 & 1.0867 \textpm{} 0.0336 & 1.0848 \textpm{} 0.0341 & 1.0776 \textpm{} 0.0389 \\
1.289 & 1.3011 \textpm{} 0.0463 & 1.2977 \textpm{} 0.0479 & 1.2880 \textpm{} 0.0538 \\
1.503 & 1.5151 \textpm{} 0.0633 & 1.5117 \textpm{} 0.0655 & 1.4989 \textpm{} 0.0736 \\
1.718 & 1.7266 \textpm{} 0.0812 & 1.7208 \textpm{} 0.0820 & 1.7022 \textpm{} 0.0907 \\
2.148 & 2.1557 \textpm{} 0.1280 & 2.1463 \textpm{} 0.1297 & 2.1176 \textpm{} 0.1439 \\
2.577 & 2.5807 \textpm{} 0.1784 & 2.5657 \textpm{} 0.1807 & 2.5252 \textpm{} 0.2052 \\
3.007 & 3.0250 \textpm{} 0.2458 & 3.0067 \textpm{} 0.2516 & \textbf{2.9472 \textpm{} 0.2762} \\
3.436 & \textbf{3.4123 \textpm{} 0.3241} & \textbf{3.3952 \textpm{} 0.3306} & 3.3242 \textpm{} 0.3619 \\
4.295 & 4.2436 \textpm{} 0.4836 & 4.2008 \textpm{} 0.4904 & 4.0825 \textpm{} 0.5280 \\
5.154 & 5.1074 \textpm{} 0.6934 & 5.0545 \textpm{} 0.7140 & 4.9037 \textpm{} 0.7743 \\
6.013 & 5.8767 \textpm{} 0.9449 & 5.8025 \textpm{} 0.9697 & 5.6116 \textpm{} 1.0619 \\
6.872 & 6.7413 \textpm{} 1.2257 & 6.6490 \textpm{} 1.2419 & 6.4272 \textpm{} 1.3127 \\
\end{tabular}
\captionof{figure}{Simulated Lifetime Measurement Results, $ \sigma_{img} $ = 5.0 mm to 25.0 mm}
$ \tau_{0} $ = 0.029 ns to 6.872 ns, $ \beta $ = 0.3c, $ N_{samples} $ = 5K, $ N_{trials} $ = 1000
\label{table:sim_lifetimes_5.0mm_to_25.0mm__0.0290ns_to_6.8720ns}
\end{table}

\begin{table}[ht]
\centering 
\begin{tabular}{c c c}
\textbf{$ \tau_{0,known} $ (ns)} & \textbf{$ \sigma_{img} $ = 35.0 mm} & \textbf{$ \sigma_{img} $ = 50.0 mm} \\ [0.5ex]
\hline
0.029 & 0.0296 \textpm{} 0.0059 & 0.0299 \textpm{} 0.0086 \\
0.072 & \textbf{0.0742 \textpm{} 0.0056} & 0.0748 \textpm{} 0.0083 \\
0.143 & 0.1470 \textpm{} 0.0055 & \textbf{0.1480 \textpm{} 0.0079} \\
0.215 & 0.2209 \textpm{} 0.0062 & 0.2226 \textpm{} 0.0089 \\
0.286 & 0.2942 \textpm{} 0.0073 & 0.2946 \textpm{} 0.0095 \\
0.358 & 0.3679 \textpm{} 0.0083 & 0.3649 \textpm{} 0.0111 \\
0.430 & 0.4390 \textpm{} 0.0101 & 0.4357 \textpm{} 0.0131 \\
0.687 & 0.6932 \textpm{} 0.0188 & 0.6873 \textpm{} 0.0246 \\
0.859 & 0.8621 \textpm{} 0.0309 & 0.8530 \textpm{} 0.0379 \\
1.074 & 1.0721 \textpm{} 0.0432 & 1.0581 \textpm{} 0.0531 \\
1.289 & 1.2790 \textpm{} 0.0603 & 1.2571 \textpm{} 0.0748 \\
1.503 & 1.4884 \textpm{} 0.0834 & 1.4639 \textpm{} 0.1003 \\
1.718 & 1.6871 \textpm{} 0.1014 & 1.6529 \textpm{} 0.1215 \\
2.148 & 2.0953 \textpm{} 0.1569 & 2.0381 \textpm{} 0.1819 \\
2.577 & \textbf{2.4877 \textpm{} 0.2262} & \textbf{2.4094 \textpm{} 0.2577} \\
3.007 & 2.8964 \textpm{} 0.2981 & 2.7962 \textpm{} 0.3409 \\
3.436 & 3.2594 \textpm{} 0.3892 & 3.1447 \textpm{} 0.4555 \\
4.295 & 4.0033 \textpm{} 0.5953 & 3.8272 \textpm{} 0.6821 \\
5.154 & 4.7842 \textpm{} 0.8281 & 4.5347 \textpm{} 0.9387 \\
6.013 & 5.4361 \textpm{} 1.1540 & 5.1376 \textpm{} 1.4534 \\
6.872 & 6.1945 \textpm{} 1.3860 & 5.7834 \textpm{} 1.5259 \\
\end{tabular}
\captionof{figure}{Simulated Lifetime Measurement Results, $ \sigma_{img} $ = 35.0 mm to 50.0 mm}
$ \tau_{0} $ = 0.029 ns to 6.872 ns, $ \beta $ = 0.3c, $ N_{samples} $ = 5K, $ N_{trials} $ = 1000
\label{table:sim_lifetimes_35.0mm_to_50.0mm__0.0290ns_to_6.8720ns}
\end{table}

\begin{table}[ht]
\centering 
\begin{tabular}{c c c c}
\textbf{$ \tau_{0,known} $ (ns)} & \textbf{$ N_{samples} $ = 500} & \textbf{$ N_{samples} $ = 1000} & \textbf{$ N_{samples} $ = 5000} \\ [0.5ex]
\hline
0.029 & 0.0300 \textpm{} 0.0142 & 0.0296 \textpm{} 0.0098 & 0.0295 \textpm{} 0.0041 \\
0.072 & 0.0736 \textpm{} 0.0144 & 0.0746 \textpm{} 0.0099 & \textbf{0.0738 \textpm{} 0.0039} \\
0.143 & 0.1444 \textpm{} 0.0155 & \textbf{0.1475 \textpm{} 0.0100} & 0.1463 \textpm{} 0.0041 \\
0.215 & \textbf{0.2164 \textpm{} 0.0177} & 0.2220 \textpm{} 0.0119 & 0.2201 \textpm{} 0.0049 \\
0.286 & 0.2880 \textpm{} 0.0219 & 0.2959 \textpm{} 0.0150 & 0.2935 \textpm{} 0.0061 \\
0.358 & 0.3611 \textpm{} 0.0272 & 0.3725 \textpm{} 0.0185 & 0.3677 \textpm{} 0.0073 \\
0.430 & \textbf{0.4357 \textpm{} 0.0332} & 0.4500 \textpm{} 0.0233 & 0.4399 \textpm{} 0.0086 \\
0.687 & 0.7231 \textpm{} 0.0714 & 0.7352 \textpm{} 0.0451 & 0.6960 \textpm{} 0.0167 \\
0.859 & 0.9243 \textpm{} 0.1043 & 0.9196 \textpm{} 0.0636 & 0.8666 \textpm{} 0.0274 \\
1.074 & 1.1838 \textpm{} 0.1614 & \textbf{1.1456 \textpm{} 0.0962} & 1.0776 \textpm{} 0.0389 \\
1.289 & 1.4371 \textpm{} 0.2280 & 1.3469 \textpm{} 0.1284 & 1.2880 \textpm{} 0.0538 \\
1.503 & 1.7081 \textpm{} 0.3111 & 1.5868 \textpm{} 0.1791 & 1.4989 \textpm{} 0.0736 \\
1.718 & 1.9790 \textpm{} 0.4143 & 1.8015 \textpm{} 0.2258 & 1.7022 \textpm{} 0.0907 \\
2.148 & 2.5362 \textpm{} 0.7025 & 2.2457 \textpm{} 0.3547 & 2.1176 \textpm{} 0.1439 \\
2.577 & 3.0681 \textpm{} 1.0121 & 2.6874 \textpm{} 0.5352 & 2.5252 \textpm{} 0.2052 \\
3.007 & 3.7695 \textpm{} 1.7073 & 3.1308 \textpm{} 0.8451 & \textbf{2.9472 \textpm{} 0.2762} \\
3.436 & 4.3022 \textpm{} 2.1353 & 3.6650 \textpm{} 1.0767 & 3.3242 \textpm{} 0.3619 \\
4.295 & 6.0336 \textpm{} 3.8683 & 4.4276 \textpm{} 1.6359 & 4.0825 \textpm{} 0.5280 \\
5.154 & 7.6861 \textpm{} 5.4939 & 5.4942 \textpm{} 2.6923 & 4.9037 \textpm{} 0.7743 \\
6.013 & 9.2424 \textpm{} 6.9364 & 6.6701 \textpm{} 3.8876 & 5.6116 \textpm{} 1.0619 \\
6.872 & 11.4505 \textpm{} 8.7428 & 7.5749 \textpm{} 4.6503 & 6.4272 \textpm{} 1.3127 \\
\end{tabular}
\captionof{figure}{Simulated Lifetime Measurement Results, $ N_{samples} $ = 500 to 5K}
$ \sigma_{img} $ = 25.0 mm, $ \tau_{0} $ = 0.029 ns to 6.872 ns, $ \beta $ = 0.3c, $ N_{trials} $ = 1000
\label{table:sim_lifetimes_500_to_5Ksamples__0.0290ns_to_6.8720ns}
\end{table}

\begin{table}[ht]
\centering 
\begin{tabular}{c c c}
\textbf{$ \tau_{0,known} $ (ns)} & \textbf{$ N_{samples} $ = 10000} & \textbf{$ N_{samples} $ = 50000} \\ [0.5ex]
\hline
0.029 & \textbf{0.0293 \textpm{} 0.0027} & \textbf{0.0289 \textpm{} 0.0012} \\
0.072 & 0.0730 \textpm{} 0.0029 & 0.0724 \textpm{} 0.0012 \\
0.143 & 0.1454 \textpm{} 0.0028 & 0.1439 \textpm{} 0.0012 \\
0.215 & 0.2185 \textpm{} 0.0035 & 0.2163 \textpm{} 0.0014 \\
0.286 & 0.2912 \textpm{} 0.0040 & 0.2871 \textpm{} 0.0017 \\
0.358 & 0.3634 \textpm{} 0.0049 & 0.3588 \textpm{} 0.0022 \\
0.430 & 0.4349 \textpm{} 0.0062 & 0.4303 \textpm{} 0.0027 \\
0.687 & 0.6904 \textpm{} 0.0122 & 0.6859 \textpm{} 0.0058 \\
0.859 & 0.8599 \textpm{} 0.0189 & 0.8562 \textpm{} 0.0081 \\
1.074 & 1.0730 \textpm{} 0.0274 & 1.0690 \textpm{} 0.0124 \\
1.289 & 1.2825 \textpm{} 0.0376 & 1.2791 \textpm{} 0.0170 \\
1.503 & 1.4925 \textpm{} 0.0501 & 1.4895 \textpm{} 0.0223 \\
1.718 & 1.6976 \textpm{} 0.0663 & 1.6970 \textpm{} 0.0298 \\
2.148 & 2.1113 \textpm{} 0.0975 & 2.1177 \textpm{} 0.0460 \\
2.577 & 2.5185 \textpm{} 0.1343 & 2.5293 \textpm{} 0.0640 \\
3.007 & 2.9292 \textpm{} 0.1933 & 2.9337 \textpm{} 0.0830 \\
3.436 & 3.3267 \textpm{} 0.2488 & 3.3376 \textpm{} 0.1123 \\
4.295 & \textbf{4.0994 \textpm{} 0.3752} & 4.1457 \textpm{} 0.1680 \\
5.154 & 4.8874 \textpm{} 0.5469 & 4.9453 \textpm{} 0.2431 \\
6.013 & 5.6760 \textpm{} 0.7411 & 5.7109 \textpm{} 0.3168 \\
6.872 & 6.4187 \textpm{} 0.9624 & \textbf{6.4951 \textpm{} 0.3992} \\
\end{tabular}
\captionof{figure}{Simulated Lifetime Measurement Results, $ N_{samples} $ = 10K to 50K}
$ \sigma_{img} $ = 25.0 mm, $ \tau_{0} $ = 0.029 ns to 6.872 ns, $ \beta $ = 0.3c, $ N_{trials} $ = 1000
\label{table:sim_lifetimes_10K_to_50Ksamples__0.0290ns_to_6.8720ns}
\end{table}

